Bias Mitigation for Machine Learning Classifiers: A Comprehensive Survey

This paper provides a comprehensive survey of bias mitigation methods for achieving fairness in Machine Learning (ML) models. We collect a total of 341 publications concerning bias mitigation for ML classifiers. These methods can be distinguished based on their intervention procedure (i.e., pre-processing, in-processing, post-processing) and the technique they apply. We investigate how existing bias mitigation methods are evaluated in the literature. In particular, we consider datasets, metrics and benchmarking. Based on the gathered insights (e.g., What is the most popular fairness metric? How many datasets are used for evaluating bias mitigation methods?), we hope to support practitioners in making informed choices when developing and evaluating new bias mitigation methods.

==> old-versions/multiple.tex <==
non binary sensitive (categorical): alabdulmohsin2022reduction, zeng2022fair2,celis2021fairadv,celis2021fair,fairn2021sharma
% multi-class





Multiple attributes: boulitsakis2022fairness,celis2021fairadv,celis2021fair,fairn2021sharma,maat





continuous sensitive attributes: jiang2022generalized




multi-class prediction: alghamdi2022beyond,alabdulmohsin2022reduction

==> old-versions/todos.tex <==
multi-class tasks?
as has already been done by x and y



Arguably, the survey might be easier to follow if it first defined what is understood by 'bias mitigation' and what types of biases will be considered. These questions stay open up until Sec. 6.
